A Preliminary Study of Fixed Flaky Tests in Rust Projects on GitHub

Prior research has extensively studied flaky tests in various domains, such as web applications, mobile applications, and other open-source projects in a range of multiple programing languages, including Java, Javascript, Python, Ruby, and more. However, little attention has been given to flaky tests in Rust -- an emerging popular language known for its safety features relative to C/C++. Rust incorporates interesting features that make it easy to detect some flaky tests, e.g., the Rust standard randomizes the order of elements in hash tables, effectively exposing implementation-dependent flakiness. However, Rust still has several sources of nondeterminism that can lead to flaky tests. We present our work-in-progress on studying flaky tests in Rust projects on GitHub. Searching through the closed Github issues and pull requests. We focus on flaky tests that are fixed, not just reported, as the fixes can offer valuable information on root causes, manifestation characteristics, and strategies of fixes. By far, we have inspected 53 tests. Our initial findings indicate that the predominant root causes include asynchronous wait (33.9%), concurrency issues (24.5%), logic errors (9.4%). and network-related problems (9.4%).

==> Tables/root-cause.tex <==
\begin{table}[h!]
\centering
\caption{Categories of flakiness root cause \yang{@Tom, should we combine Async Wait "Tweak durations"  and "Tweak Durations" as one item? also "Wait/Join" and "Wait"?}
\tom{Yeah, I would combine 'tweak durations' together. Also, all 'wait' items could be combined. We're not pulling from a predefined set of labels/categories, so the nomenclature is evolving as we do the investigation.}}
\begin{tabular}{@{}lrlr@{}}
\toprule
\textbf{Root Cause (Percent)} & \textbf{Total} & \textbf{Root Cause (Percent)} & \textbf{Total} \\ \midrule
\addlinespace
\textbf{Async Wait (33.9\%)} & 18 & \textbf{Concurrency (24.5\%)} & 13 \\
Wait/Join & 5 & Robustness & 4 \\
Wait & 2 & Retry & 2 \\
Sleep & 2 & Channels & 1 \\
Channels & 1 & Lock & 1 \\
Configuration & 1 & Race Condition & 1 \\
Unknown state & 1 & Non-deterministic environment & 1 \\
Tweak durations & 1 & Reorder initialization & 1 \\
Tweak Durations & 1 & Shared state & 1 \\
Retry & 1 & Atomics & 1 \\
Deadlock & 1 & & \\
Increase timeout & 1 & & \\
Wait/Lock & 1 & & \\
\addlinespace
\textbf{Logic (9.4\%)} & 5 & \textbf{Network (9.4\%)} & 5 \\
Off by one & 2 & Certs & 1 \\
Inverted Conditional & 1 & Connection loss & 1 \\
Deserialization & 1 & Empty header & 1 \\
Sorting & 1 & Retry & 1 \\
& & Reused resource (port) & 1 \\
\addlinespace
\textbf{I/O (5.6\%)} & 3 & \textbf{Randomness (5.7\%)} & 3 \\
Flush & 1 & Ranges & 1 \\
Temp Files & 1 & RNG & 1 \\
Resource limit & 1 & Weighting & 1 \\
\addlinespace
\textbf{Time (3.8\%)} & 2 & \textbf{Unordered data (5.7\%)} & 3 \\
Inconsistent clock & 1 & Sorting & 2 \\
Off by one & 1 & Non-deterministic environment & 1 \\
\addlinespace
\textbf{Environment (1.9\%)} & 1 & & \\
Shared libraries & 1 & & \\
\bottomrule
% Total & & & 53\\ \hline
\end{tabular}
% \label{root-cause}
\end{table}

